Private Hierarchical Governance for Encrypted Messaging

The increasing harms caused by hate, harassment, and other forms of abuse online have motivated major platforms to explore hierarchical governance. The idea is to allow communities to have designated members take on moderation and leadership duties; meanwhile, members can still escalate issues to the platform. But these promising approaches have only been explored in plaintext settings where community content is public to the platform. It is unclear how one can realize hierarchical governance in the huge and increasing number of online communities that utilize end-to-end encrypted (E2EE) messaging for privacy. We propose private hierarchical governance systems. These should enable similar levels of community governance as in plaintext settings, while maintaining cryptographic privacy of content and governance actions not reported to the platform. We design the first such system, taking a layered approach that adds governance logic on top of an encrypted messaging protocol; we show how an extension to the message layer security (MLS) protocol suffices for achieving a rich set of governance policies. Our approach allows developers to rapidly prototype new governance features, taking inspiration from a plaintext system called PolicyKit. We build a prototype E2EE messaging system called MlsGov that supports content-based community and platform moderation, elections of community moderators, votes to remove abusive users, and more.

==> snippets.tex <==



First, platforms are transnational organizations, spanning numerous languages and cultures, while platform-level moderators often lack the linguistic or cultural knowledge to properly pass judgement on all the content they review (cite Arabic content moderation). Second, many forms of platform-driven moderation rely on being able to see content in the clear. Examples of this include text filters, content block-lists, etc. This poses a challenge to end-to-end encrypted (E2EE) platforms such as WhatsApp, Signal, and Keybase. Recent work has explored content-oblivious forms of moderation (cite Riana's paper), however it remains clear that certain important moderation functionalities require access to plaintext content, which poses an immense privacy risk to the users of E2EE platforms. Third, platform-driven moderation is an often opaque and brittle process and is difficult for many users to understand \cite{UserInterpMod}.

A solution for online communities that partially addresses these concerns  is platform-provided community moderation and governance tools. Examples of these tools include the Reddit Auto-moderator (cite), Matrix power levels (cite), and user-configured Discord moderation-bots (cite, check). Community members, who have a deep understanding of the norms within their community, perform moderation, instead of relying on disconnected external platform moderators. Although these tools are useful, they are limited in functionality and difficult to extend. Furthermore, some of these platform-provided tools (e.g. AutoMod and mod bots) rely on plaintext-access, making them unsuitable for E2EE communities.

The limits of platform-provided moderation functionality have prompted Twitter users to resort to third-party services such as collaborative blocklists \cite{TwitterBotBlocklists}, which allow users to subscribe to curated user blocklists, enabling moderation functionality on top of what Twitter provides.

\subsection{Types of Communities}
In considering different designs for private governance, it becomes useful to consider the space of communities that we wish to design for and against in addition to how transparency, accountability, security, and privacy trade off with one another for those communities. Transparency in its most extreme form, for instance, is directly at odds with privacy.

We propose modeling communities by examining the alignment between users, community moderators, platform moderators, and society. This modeling will necessarily be imperfect and vague, however, it provides a rudimentary framework for describing different community archetypes and how they might interact with various governance designs. We use the term \textit{alignment matrix} to refer to a diagram that shows the alignments between all possible pairs of users (U), community moderators (C), platform moderators (M), and society (S). The alignment between a group and itself expresses how much conflict and disagreement occurs within the group. We will express alignments as values between 0 and 1.

\begin{table}[h]
\begin{minipage}{0.5\textwidth}
\begin{tabular}{lllll}
           & \textbf{U} & \textbf{C} & \textbf{P} & \textbf{S} \\
\textbf{U} & 1          & 1          & 1          & 1          \\
\textbf{C} & --         & 1          & 1          & 1          \\
\textbf{P} & --         & --         & 1          & 1          \\
\textbf{S} & --         & --         & --         & 1         
\end{tabular}
\centering
\caption{A wholesome community.}
\label{table:wholesome}
\end{minipage}%
\begin{minipage}{0.5\textwidth}
\begin{tabular}{lllll}
           & \textbf{U} & \textbf{C} & \textbf{P} & \textbf{S} \\
\textbf{U} & 1          & 1          & 0          & 0          \\
\textbf{C} & --         & 1          & 0          & 0          \\
\textbf{P} & --         & --         & 1          & 1          \\
\textbf{S} & --         & --         & --         & 1         
\end{tabular}
\centering
\caption{An extremist community.}
\label{table:extremist}
\end{minipage}
\end{table}

\begin{table}[h]
\begin{minipage}{0.5\textwidth}
\begin{tabular}{lllll}
           & \textbf{U} & \textbf{C} & \textbf{P} & \textbf{S} \\
\textbf{U} & 0.25          & 1          & 1          & 1          \\
\textbf{C} & --         & 1          & 1          & 1          \\
\textbf{P} & --         & --         & 1          & 1          \\
\textbf{S} & --         & --         & --         & 1         
\end{tabular}
\centering
\caption{A community with abusive users.}
\label{table:abusiveUsers}
\end{minipage}%
\begin{minipage}{0.5\textwidth}
\begin{tabular}{lllll}
           & \textbf{U} & \textbf{C} & \textbf{P} & \textbf{S} \\
\textbf{U} & 1          & 0          & 1          & 1          \\
\textbf{C} & --         & 1          & 0          & 0          \\
\textbf{P} & --         & --         & 1          & 1          \\
\textbf{S} & --         & --         & --         & 1         
\end{tabular}
\centering
\caption{Moderators abusive toward users}
\label{table:abusiveMods}
\end{minipage}
\end{table}


==> table-security-analysis.tex <==
\begin{figure*}[t]
    \centering
    \scriptsize
    \begin{tabular}{p{0.1\textwidth}p{0.2\textwidth}p{0.3\textwidth}p{0.3\textwidth}} \textbf{Category}
    & \textbf{Attack Type}    & \textbf{Description}
    & \textbf{Detection/ Mitigation}
    \\\toprule \multirow{5}{*}{Integrity}       & Impersonation
    & A malicious user impersonates a moderator
    & Authenticity guarantees of messaging layer
    \\
    & Policy violation & A malicious user performs an unauthorized
     action & Authenticity and consensus of
                                     governance messages \\

    & Discrepancy in governance state & A malicious user attempts to partition
    governance state among existing members & Detected by transcript hash\\
    & Discrepancy in governance state & A malicious user invites a new
    member and provides them with an incorrect group state & Detected by
    governance state hash in Accept message \\
    & Vote suppression & A malicious DS attempts to prevent a client's votes
    from being counted & Detected by transcript hash\\
                                                            \midrule
    
    \multirow{1}{*}{Accountability}  & Report evasion      & A malicious user generates an un-reportable message                                             & Same verification process for message recipient and report recipient   \\ 
    & Fake reports      & A malicious user frames another user                                                    & Existential unforgeability of digital signature    \\\midrule  
    \multirow{2}{*}{Confidentiality} 
    
    
    & Inferring content of governance state & A malicious DS attempts to learn governance state & Updates to the governance state and group state announcements are encrypted. \\
    & Inferring content of un-reported text messages     & A malicious DS
    attempts to learn message content
    & Encryption of message and reporting signature
    \\
    & Inferring the content of user votes & A malicious DS attempting to
    learn a user vote & Votes are encrypted \\
    & Inferring the outcome of a vote & A malicious DS attempting to learn
    vote outcome & Votes are encrypted and aggregated on client devices \\
    \bottomrule             
    \end{tabular}
    \caption{An overview of various attacks and how our system mitigates and/or provides eventual detection for them.}
    \label{fig:attacks}
\end{figure*}

